Can We Solve 3D Vision Tasks Starting from A 2D Vision Transformer?

Vision Transformers (ViTs) have proven to be effective, in solving 2D image understanding tasks by training over large-scale image datasets; and meanwhile as a somehow separate track, in modeling the 3D visual world too such as voxels or point clouds. However, with the growing hope that transformers can become the "universal" modeling tool for heterogeneous data, ViTs for 2D and 3D tasks have so far adopted vastly different architecture designs that are hardly transferable. That invites an (over-)ambitious question: can we close the gap between the 2D and 3D ViT architectures? As a piloting study, this paper demonstrates the appealing promise to understand the 3D visual world, using a standard 2D ViT architecture, with only minimal customization at the input and output levels without redesigning the pipeline. To build a 3D ViT from its 2D sibling, we "inflate" the patch embedding and token sequence, accompanied with new positional encoding mechanisms designed to match the 3D data geometry. The resultant "minimalist" 3D ViT, named Simple3D-Former, performs surprisingly robustly on popular 3D tasks such as object classification, point cloud segmentation and indoor scene detection, compared to highly customized 3D-specific designs. It can hence act as a strong baseline for new 3D ViTs. Moreover, we note that pursing a unified 2D-3D ViT design has practical relevance besides just scientific curiosity. Specifically, we demonstrate that Simple3D-Former naturally enables to exploit the wealth of pre-trained weights from large-scale realistic 2D images (e.g., ImageNet), which can be plugged in to enhancing the 3D task performance "for free".

==> tables/ablation_1st_layer_attention.tex <==
\begin{table}[ht]
\caption{Performance under different 2D ViT backbone, with group embedding scheme and evaluated in OA. (\%)}
\begin{center}
\label{tab:ablation:pretrain}
\begin{threeparttable}
\resizebox{0.999\linewidth}{!}{
\begin{tabular}{c|c|c}
\hline 
{\bf Backbone Name}  &{\bf ShapeNetV2}  &{\bf ModelNet40} \\ \hline 
DeiT-tiny  & 82.8 &  \\ \hline 
DeiT-small   & 83.5& \\ \hline 
%Finetuning First Layer First &  \\ \hline 
DeiT-base  &  84.3&  \\ \hline 
\end{tabular}
}
\end{threeparttable}
\end{center}
\end{table}



==> tables/ablation_AMSoftmax.tex <==
\begin{table}[ht]
\caption{Ablation Study for Additive Margin Softmax Layer}
\label{tab:ablation:tricks}
\begin{center}
\begin{tabular}{c|c}
\multicolumn{1}{c}{\bf Model}\vline  &\multicolumn{1}{c}{\bf result} \\
\hline
Linear head only     &  85.6  \\
With AMSoftmax        &  85.4 \\
AMSoftmax+Class reweigt &  \\
\end{tabular}
\end{center}
\end{table}


==> tables/classification_scanobjectNN.tex <==
\begin{table}[t]
\begin{center}
\caption{Baseline Comparison in ScanobjectNN(PB-T50-RS) Dataset (using 1024 points)}
\label{tab:classification:scanobjectnn}
\begin{threeparttable}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{c|c|c}
\hline
\textbf{Method} & \textbf{Modality} & \textbf{PB-T50-RS} OA. (\%) \\ 
\hline
PointNet & Point &  68.0\\ \hline
PointNet++ & Point & 77.9\\ \hline
DGCNN & Voxel  &  78.1\\ \hline
Point Transformer & Point &  81.2 \\ \hline
Point-BERT  & Point &  \textbf{83.1} \\ \hline
% Simple3D-Former (deIT-Tiny)  & Point &  81.2 \\ \hline
Simple3D-Former (ours)  & Point &  \textbf{83.1} \\  \hline
\end{tabular}}
\end{threeparttable}
\vspace{-1em}
\end{center}
\end{table}

